DES16C3cje: A low-luminosity, long-lived supernova

We present DES16C3cje, a low-luminosity, long-lived type II supernova (SN II) at redshift 0.0618, detected by the Dark Energy Survey (DES). DES16C3cje is a unique SN. The spectra are characterized by extremely narrow photospheric lines corresponding to very low expansion velocities of $\lesssim1500$ km s$^{-1}$, and the light curve shows an initial peak that fades after 50 days before slowly rebrightening over a further 100 days to reach an absolute brightness of M$_r\sim -15.5$ mag. The decline rate of the late-time light curve is then slower than that expected from the powering by radioactive decay of $^{56}$Co but is comparable to that expected from accretion power. Comparing the bolometric light curve with hydrodynamical models, we find that DES16C3cje can be explained by either i) a low explosion energy (0.11 foe) and relatively large $^{56}$Ni production of 0.075 M$_{\odot}$ from a $\sim15$ M$_{\odot}$ red supergiant progenitor typical of other SNe II, or ii) a relatively compact $\sim40$ M$_{\odot}$ star, explosion energy of 1 foe, and 0.08 M$_{\odot}$ of $^{56}$Ni. Both scenarios require additional energy input to explain the late-time light curve, which is consistent with fallback accretion at a rate of $\sim0.5\times{10^{-8}}$ M$_{\odot}$ s$^{-1}$.

==> table_spec.tex <==
\begin{table*}
\centering
\small
\caption{Spectroscopy of DES16C3cje}
\label{spec}
\begin{tabular}[t]{ccccccccccc}
\hline
UT date		&	MJD    & Phase	&  Telescope    &  Range	&  Grism/Grating/	\\
		    & (days)   & (days) & + Instrument	&  (\AA)	&     Arm          \\
\hline
\hline               
20161127    & 57720.0  &  49    &  AAT+AAOmega   &  3750 -- 9000  & 580V+385R  \\
20170102    & 57755.7  &  85    &  Gemini+GMOS-S &  5700 -- 7500  & R400-G5305   \\
20170129    & 57782.0  &  112   &  VLT+XSHOOTER  &  3100 -- 10400 & UV/VIS/NIR   \\
20170221    & 57805.0  &  135   &  VLT+XSHOOTER  &  3100 -- 10400 & UV/VIS/NIR   \\
20170731    & 57965.3  &  295   &  VLT+FORS2     &  4300 -- 9500  & 300V+GG435       \\
20171116    & 58074.2  &  403   &  VLT+XSHOOTER  &  3600 -- 9600  & UV/VIS/NIR   \\
\hline
\hline
\end{tabular}
%\begin{list}{}{}
%\item Note that \\
%\end{list}
\end{table*}

